Improving Text Auto-Completion with Next Phrase Prediction

Language models such as GPT-2 have performed well on constructing syntactically sound sentences for text auto-completion task. However, such models often require considerable training effort to adapt to specific writing domains (e.g., medical). In this paper, we propose an intermediate training strategy to enhance pre-trained language models' performance in the text auto-completion task and fastly adapt them to specific domains. Our strategy includes a novel self-supervised training objective called Next Phrase Prediction (NPP), which encourages a language model to complete the partial query with enriched phrases and eventually improve the model's text auto-completion performance. Preliminary experiments have shown that our approach is able to outperform the baselines in auto-completion for email and academic writing domains.

==> paper/030related.tex <==

Towards enhancing the performance of Pre-trained Language Models, recent works focus on further training on data-rich intermediate task before fine-tuning it on a target task~\cite{pruksachatkun-etal-2020-intermediate}, incorporating knowledge base during pre-training~\cite{Xiong2020Pretrained} and exploiting external knowledge with specific architecture~\cite{peters-etal-2019-knowledge}. 
Compared to these works, our approach can directly improve the suggestion ability without relying on external knowledge bases.
